Text Revealer: Private Text Reconstruction via Model Inversion Attacks against Transformers

Text classification has become widely used in various natural language processing applications like sentiment analysis. Current applications often use large transformer-based language models to classify input texts. However, there is a lack of systematic study on how much private information can be inverted when publishing models. In this paper, we formulate \emph{Text Revealer} -- the first model inversion attack for text reconstruction against text classification with transformers. Our attacks faithfully reconstruct private texts included in training data with access to the target model. We leverage an external dataset and GPT-2 to generate the target domain-like fluent text, and then perturb its hidden state optimally with the feedback from the target model. Our extensive experiments demonstrate that our attacks are effective for datasets with different text lengths and can reconstruct private texts with accuracy.

==> 4_related.tex <==
Model inversion attack was first proposed in ~\cite{fredrikson2015model}. Several work~\cite{Zhang_2020_CVPR, zhang2018collaborative} in computer vision domain  further developed it and construct attacks for deep neural networks. ~\cite{Zhang_2020_CVPR} proposed to use a generative model to help the adversary reveal more sensitive attributes.  ~\cite{wang2021variational} treats the model inversion attack as a variational inference problem and trains generative models to invert the private dataset distribution. In natural language processing field, KART~\cite{nakamura2020kart}, ~\cite{pan2020privacy} and ~\cite{lehman2021does} explore invert tabular data with sensitive attributes from the medical datasets. However, they follow a fill-in-blank scheme and it's hard to synthesis sentences with fluency from scratch.


